EigenFairing: 3D Model Fairing using Image Coherence

A surface is often modeled as a triangulated mesh of 3D points and textures associated with faces of the mesh. The 3D points could be either sampled from range data or derived from a set of images using a stereo or Structure-from-Motion algorithm. When the points do not lie at critical points of maximum curvature or discontinuities of the real surface, faces of the mesh do not lie close to the modeled surface. This results in textural artifacts, and the model is not perfectly coherent with a set of actual images -- the ones that are used to texture-map its mesh. This paper presents a technique for perfecting the 3D surface model by repositioning its vertices so that it is coherent with a set of observed images of the object. The textural artifacts and incoherence with images are due to the non-planarity of a surface patch being approximated by a planar face, as observed from multiple viewpoints. Image areas from the viewpoints are used to represent texture for the patch in Eigenspace. The Eigenspace representation captures variations of texture, which we seek to minimize. A coherence measure based on the difference between the face textures reconstructed from Eigenspace and the actual images is used to reposition the vertices so that the model is improved or faired. We refer to this technique of model refinement as EigenFairing, by which the model is faired, both geometrically and texturally, to better approximate the real surface.

==> 03exper.tex <==
\section{Experiments}

\begin{figure}
        \figdef{FigEigFSmooth}
        \caption{At each iteration for updating the position of the vertex, a coarse-to-fine strategy is used to calculate the 3D vertex displacement. The arrows show the displacement (magnified $\times$10) for two views in the $5$-th iterative step. }
        \label{fig:eigFSmooth}
\end{figure}

\begin{figure}
  \begin{center}
  \setcounter{subfigure}{0}
  \subfigure[Path of vertex $A$ superimposed on images shown in Figure \ref{fig:eigFInit}. $A^0_i$ and $A^0_j$ correspond to the initial position of the vertex. $A_i$ and $A_j$ correspond to the 3D point the vertex converges to.] 
  { \inserteps[scale=1.1]{FIGURES/eigFPath.eps}
    \label{fig:eigFPath1} }
   \end{center}

 \begin{center}
  \setcounter{subfigure}{1}
  \subfigure[Error in Position of Vertex] 
  { \inserteps[scale=0.60]{FIGURES/eigFG1pos.eps}
    \label{fig:eigFG1} }
  \setcounter{subfigure}{2}
  \subfigure[Residual Pixel-Error of Faces sharing the Vertex] 
  { \inserteps[scale=0.60]{FIGURES/eigFG2err.eps} 
    \label{fig:eigFG4} }
 \end{center}

% \begin{center}
% \setcounter{subfigure}{2}
% \subfigure[Pixel Error Norm and  $\sigma$] 
% { \inserteps[scale=0.60]{FIGURES/eigFG1pos.eps} 
%   \label{fig:eigFG3} }
% \setcounter{subfigure}{5}
% \subfigure[First Five Eigenvalues for Face ADB] 
% { \inserteps[scale=0.60]{FIGURES/eigFG2err.eps} 
%   \label{fig:eigFG6} }
% \end{center}
 
 \caption{The process of fairing the mesh by relocating vertex $A$ based on texture of faces common to the vertex.}
 \label{fig:eigFGraphs}
\end{figure}


==> 04discu.tex <==
\section{Discussion}

For large values of $\sigma$, 
$\ddot{\rho}(e_c)=\frac{2\sigma(\sigma-3e_c^2)}{(\sigma+e_c^2)^3}$ 
is positive and therefore the Hessian is positive-definite and the rate of local convergence 
is quadratic. The secant approximation to the Hessian gives linear rate of convergence 
and is only accurate for small error residuals. 
A robust error norm such as the Geman-McClure norm has the effect of reducing the size of 
large residuals, and one might expect that this would increase the reliability of the 
Gauss-Newton method.  
\begin{figure*}
        %\figdef{FigEigFHamMesh}
        \inserteps[scale=2.1XS]{FIGURES/eigFHamMesh.eps}
 	\caption{On the top row is the triangulated mesh with initial position of the vertices as observed from different views. On the bottom is the faired mesh.}
        \label{fig:eigFHamMesh}
\end{figure*}

\begin{figure}
        \figdef{FigEigFHamResults}
        \caption{Two views of the texture-mapped mesh for the initial (top) and final position (bottom) of the vertices. Notice the textural artifacts in the views on the top row.}
        \label{fig:eigFHamResults}
\end{figure}
